IntelliAV: Building an Effective On-Device Android Malware Detector

The importance of employing machine learning for malware detection has become explicit to the security community. Several anti-malware vendors have claimed and advertised the application of machine learning in their products in which the inference phase is performed on servers and high-performance machines, but the feasibility of such approaches on mobile devices with limited computational resources has not yet been assessed by the research community, vendors still being skeptical. In this paper, we aim to show the practicality of devising a learning-based anti-malware on Android mobile devices, first. Furthermore, we aim to demonstrate the significance of such a tool to cease new and evasive malware that can not easily be caught by signature-based or offline learning-based security tools. To this end, we first propose the extraction of a set of lightweight yet powerful features from Android applications. Then, we embed these features in a vector space to build an effective as well as efficient model. Hence, the model can perform the inference on the device for detecting potentially harmful applications. We show that without resorting to any signatures and relying only on a training phase involving a reasonable set of samples, the proposed system, named IntelliAV, provides more satisfying performances than the popular major anti-malware products. Moreover, we evaluate the robustness of IntelliAV against common obfuscation techniques where most of the anti-malware solutions get affected.

==> sections/background.tex <==
\section{Background} \label{sect:background}
To better understand the whole GCM mechanism and how this service can be misused by an attacker, in this section we first discuss how GCM works, and then report an example of a dissected GCM badware.

\subsection{Google Cloud Messaging}
Google announced Cloud-to-Device-Messaging (C2DM) system in Google I/O 2010 as a push mechanism 
for Android applications. It gradually became more efficient and was renamed to Google Cloud Messaging (GCM) in Google I/O 2012\footnote{https://developers.google.com/android/c2dm/}.
The new version of GCM has received a lot of improvement such as being cross-platform 
(support iOS and Chrome) as well as having simplified APIs, and was re-branded to 
Firebase Cloud Messaging (FCM) in Google I/O 2016. 
Based on reports presented in Google I/O 2016, Google receives around 2 millions queries per second, 
and more than 1 million apps have been registered by GCM. 

Figure~\ref{fig:GCM} shows how the whole mechanism works. First, the application needs to register
itself to the GCM servers. After it receives a registration ID from the GCM servers, it sends the registration ID to its server for further communications. 
Whenever the App server needs to notify its clients, it can send data up to 4KB to a specific registration ID or 
a group of IDs through the GCM servers. When no Internet access is available on the client device, the messages accumulate in a queue on the server, and synchronize with the client device when it returns online. 
The connection protocol between App servers and GCM servers can be either HTTP or 
XMPP\footnote{It is a persistent, asynchronous, and bidirectional connection.}.
GCM provides a set of APIs for sending messages from servers to applications efficiently and reliably. 
These APIs can be categorized into 4 classes:
\textit{Registration}, an application needs a registration ID to communicate;
\textit{Send}, server can send messages to a particular device (registration ID);
\textit{Multi-cast}, it is possible to send messages to thousands recipients with a single request;
\textit{Time to live}, setting TTL on each request allows GCM to know when to expire a message.

\input{images/gcm.tex}

\subsection{GCM Badware}
We describe the two possible cases of use of GCM in badware, namely, bot clients and adware, to better motivate how modeling GCM services can be beneficial in a detection system.

\textbf{Botnet.} Many Android bot clients use unencrypted channels like HTTP to accept messages 
from command and control bot masters \cite{Aresu:2015:http}.
However, the bot masters can also take advantage of secure popular 
public services for attacks. Three types of secure services that are frequently exploited by Android 
bot clients are email over SSL, GCM, and social networks (e.g., Twitter) \cite{Trendmicro:2014:AMSSL}. 
By using these services, attackers can launch C\&C attacks in a secure way, which is not easily 
detectable by normal TCP and HTTP traffic analysis. Furthermore, defenders cannot employ simple server
blacklisting to mitigate such threats, because the email or GCM servers are used for badware as well as benign applications.

To better explain the misuse of GCM for C\&C 
purposes, Figure~\ref{fig:gcm-mal} presents a part of a decompiled \texttt{Maxit} backdoor sample
\footnote{Badware's MD5: 157febb16d16e8bcb5ba6564a2f7d320}. It shows that 
after the bot client receives a GCM message, the content of the message is accessible through
the \texttt{Intent} parameter of \texttt{onMessage} method (step 1). Then, the data is retrieved from the \texttt{Intent} by \texttt{getExtras} method and passed to
\texttt{Process\_Message} method which separates the command (step 2, 3) and executes 
consequent actions based on the command. After doing the action, the bot client sends an SMS to the attacker through \texttt{sendTextMessage} (step 5), which is located in \texttt{SendSMSNow} method (step 4). The SMS contains
the received original GCM message, a retrieved data from \texttt{SharedPreferences} (e.g., IMEI ) and the package name, which are split by \texttt{``|"}. 
Since the attacker might receive many SMS
messages, one probable answer to why the bot client sends the original GCM message along with 
the other information is to make the content of SMS easier for attacker to comprehend.
It is obvious that as the received GCM message goes directly to \texttt{sendTextMessage}, 
there is an explicit data flow between the \texttt{Intent} parameter of \texttt{onMessage} 
in \texttt{GCMIntentService} and the \texttt{sendTextMessage} API. However, if the action is decided based 
on an \texttt{if} condition, the flow would be implicit. For example, in (step +), if the command
equals to \texttt{IMEI}, the badware retrieves the identification number of the device from \texttt{SharedPreferences} so that
there is an implicit flow between \texttt{onMessage} and \texttt{getSharedPreferences}.

\begin{figure*}[!htbp]
   \centering
	\includegraphics[trim={8cm 5.5cm 7cm 7.3cm},clip,width=0.95\textwidth]{Images/gcm-mal.pdf}
    \caption{A part of Backdoor.AndroidOS.Maxit.a badware, which uses GCM for C\&C.}
     \label{fig:gcm-mal}
\end{figure*}

\textbf{Adware.} Opposite of the aforementioned deliberate misuse of GCM, it might happen that 
GCM is exploited by badware indirectly. For instance, many adlibraries such as 
Revmob, Airpush, Leadbolt, Domob and Cauly \cite{mobadlib} use GCM to notify 
users whenever a new advertisement has to be shown. As the purpose of adware is showing advertisement to  receive benefits, these adlibraries might be embedded 
in adware to display unwanted ads when the user is online.
As a result, GCM is unintentionally exploited as part of such malicious activities.


